FIFO Queueing Policies for Packets with Heterogeneous Processing

We consider the problem of managing a bounded size First-In-First-Out (FIFO) queue buffer, where each incoming unit-sized packet requires several rounds of processing before it can be transmitted out. Our objective is to maximize the total number of successfully transmitted packets. We consider both push-out (when the policy is permitted to drop already admitted packets) and non-push-out cases. In particular, we provide analytical guarantees for the throughput performance of our algorithms. We further conduct a comprehensive simulation study which experimentally validates the predicted theoretical behaviour.

==> graphs/FIFO.k10C1.tex <==
\addplot [const plot,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.902043729185197)
(3, 0.912996361947519)
(4, 0.931106511460094)
(5, 0.946722509928215)
(6, 0.958200445937174)
(7, 0.965622210738949)
(8, 0.972441055784561)
(9, 0.976881271295418)
(10, 0.980742701089558)
(11, 0.983372119210269)
(12, 0.985831175167962)
(13, 0.98756755742381)
(14, 0.989378671020286)
(15, 0.990758115969225)
(16, 0.991752828807866)
(17, 0.992691142114596)
(18, 0.993610673271786)
(19, 0.994248721677534)
(20, 0.99472721302247)
(21, 0.995318290566215)
(22, 0.995749870994981)
(23, 0.99605010085847)
(24, 0.99658488530281)
(25, 0.996810057700427)
(26, 0.99707275883098)
(27, 0.997316695595065)
(28, 0.99751372144298)
(29, 0.997748276023831)
(30, 0.997898390955575)
(31, 0.998057888070554)
(32, 0.998151709902894)
(33, 0.998320589201107)
(34, 0.998461321949618)
(35, 0.998564525965192)
(36, 0.99863020124783)
(37, 0.998724023080171)
(38, 0.998789698362809)
(39, 0.998845991462213)
(40, 0.998958577661022)
};


==> graphs/FIFO.k3C1.tex <==
\addplot [const plot,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.930420629672957)
(3, 0.941505452416384)
(4, 0.957553600945935)
(5, 0.96990980156344)
(6, 0.978950909484105)
(7, 0.984795258426561)
(8, 0.989042066456114)
(9, 0.99212853720482)
(10, 0.9944462123168)
(11, 0.995833183231865)
(12, 0.996907909746989)
(13, 0.997778498264827)
(14, 0.998354887904223)
(15, 0.998811196368745)
(16, 0.999087383070956)
(17, 0.999321541361961)
(18, 0.999531683417991)
(19, 0.999597728064171)
(20, 0.999711805180302)
(21, 0.999777849826483)
(22, 0.999831886355176)
(23, 0.999867910707638)
(24, 0.999885922883869)
(25, 0.999909939118844)
(26, 0.999939959412563)
(27, 0.999933955353819)
(28, 0.999933955353819)
(29, 0.999927951295076)
(30, 0.999927951295076)
(31, 0.999933955353819)
(32, 0.999933955353819)
(33, 0.999933955353819)
(34, 0.999933955353819)
(35, 0.999927951295076)
(36, 0.999921947236332)
(37, 0.999921947236332)
(38, 0.999921947236332)
(39, 0.999915943177588)
(40, 0.999915943177588)
};


==> graphs/FIFO.k40C1.tex <==
\addplot [const plot,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.889350120420591)
(3, 0.892118191271919)
(4, 0.913715963507987)
(5, 0.932486017558138)
(6, 0.944502906826298)
(7, 0.953913163240712)
(8, 0.961274568809864)
(9, 0.966387709862011)
(10, 0.970595307615678)
(11, 0.974262559664847)
(12, 0.976964141648214)
(13, 0.979509181396945)
(14, 0.981296544150451)
(15, 0.982723420316709)
(16, 0.983960613442207)
(17, 0.985334225286883)
(18, 0.986502015264557)
(19, 0.987257541717402)
(20, 0.988149951982439)
(21, 0.988510477758343)
(22, 0.989145346045682)
(23, 0.989659961932198)
(24, 0.990123287436341)
(25, 0.990843621399177)
(26, 0.991426758800432)
(27, 0.99171839100168)
(28, 0.992130034463248)
(29, 0.992438790206433)
(30, 0.992713119813456)
(31, 0.99300471495928)
(32, 0.993330590131331)
(33, 0.993484895243974)
(34, 0.993776467159292)
(35, 0.993982203782125)
(36, 0.994102216812111)
(37, 0.994290808716375)
(38, 0.994479495268139)
(39, 0.994616650665204)
(40, 0.9948738170347)
};


==> graphs/FIFO.k5C1.tex <==
\addplot [const plot,color=blue,mark=+,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.916772210552329)
(3, 0.929236840561)
(4, 0.945586247280035)
(5, 0.958380064992954)
(6, 0.967216171061029)
(7, 0.973441125082348)
(8, 0.978089915779983)
(9, 0.981581883726253)
(10, 0.984510648035584)
(11, 0.986872399147707)
(12, 0.988553493293677)
(13, 0.990141056529852)
(14, 0.991428060768543)
(15, 0.992493404920037)
(16, 0.993422839903344)
(17, 0.994323624873104)
(18, 0.994845545078246)
(19, 0.995531852529686)
(20, 0.996017986974457)
(21, 0.996582760814704)
(22, 0.996782933821374)
(23, 0.997311962481859)
(24, 0.997605072955912)
(25, 0.997976822825442)
(26, 0.998141250652349)
(27, 0.998305678479257)
(28, 0.998477255342117)
(29, 0.998641683169025)
(30, 0.998841856175695)
(31, 0.998920495571172)
(32, 0.999092072434032)
(33, 0.999235053153082)
(34, 0.999292245440702)
(35, 0.99937088483618)
(36, 0.999449524231657)
(37, 0.999478120375467)
(38, 0.999585355914755)
(39, 0.999585355914755)
(40, 0.999613952058565)
};


==> graphs/GreedyNP.k10C1.tex <==
\addplot [const plot,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 0.500380007461965)
(2, 0.374469933599487)
(3, 0.3514977939469)
(4, 0.343527468145307)
(5, 0.341992812066672)
(6, 0.340154102339759)
(7, 0.340367360360784)
(8, 0.340989117268707)
(9, 0.340501422041169)
(10, 0.33940520097225)
(11, 0.34061819683207)
(12, 0.340586645648013)
(13, 0.339504203573037)
(14, 0.340023269342641)
(15, 0.340823794332896)
(16, 0.3383029029292)
(17, 0.340692230468274)
(18, 0.341448997973429)
(19, 0.341023596190834)
(20, 0.34168973120045)
(21, 0.339616268705728)
(22, 0.339494300323685)
(23, 0.339860205469813)
(24, 0.340779659426749)
(25, 0.339588122156026)
(26, 0.340104142233898)
(27, 0.339522446873387)
(28, 0.341136182389642)
(29, 0.338058826288877)
(30, 0.339222217009898)
(31, 0.340451283013557)
(32, 0.339456771590749)
(33, 0.339935262935685)
(34, 0.340760895060281)
(35, 0.343115823052024)
(36, 0.339616268705728)
(37, 0.340732748510578)
(38, 0.341323826054323)
(39, 0.338865694047005)
(40, 0.338696814748792)
};


==> graphs/GreedyNP.k3C1.tex <==
\addplot [const plot,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 0.773059170410164)
(2, 0.636475764203245)
(3, 0.610249810934107)
(4, 0.603178050457885)
(5, 0.601473241130487)
(6, 0.600415695509047)
(7, 0.600575282086388)
(8, 0.599906332184502)
(9, 0.599612130818788)
(10, 0.600559581634675)
(11, 0.601072324891627)
(12, 0.600826158483135)
(13, 0.600628024544592)
(14, 0.600153703903839)
(15, 0.600808146306903)
(16, 0.601720763235947)
(17, 0.600063643022683)
(18, 0.600700073249517)
(19, 0.599913541554091)
(20, 0.601156381714039)
(21, 0.601342507535094)
(22, 0.600628024544592)
(23, 0.601192406066501)
(24, 0.599823480672935)
(25, 0.601108349244089)
(26, 0.600303805372432)
(27, 0.600868186894341)
(28, 0.601684738883485)
(29, 0.599889525319116)
(30, 0.60000960649399)
(31, 0.601114353302833)
(32, 0.601378531887556)
(33, 0.601282466947657)
(34, 0.601186402007757)
(35, 0.601042304597908)
(36, 0.600561979898411)
(37, 0.600483927134743)
(38, 0.600832162541878)
(39, 0.600730093543235)
(40, 0.601858856587053)
};


==> graphs/GreedyNP.k40C1.tex <==
\addplot [const plot,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 0.268536410313035)
(2, 0.191106498795794)
(3, 0.176659375336178)
(4, 0.168548358908036)
(5, 0.168395352461429)
(6, 0.168354408542792)
(7, 0.167320869056227)
(8, 0.169363575395938)
(9, 0.169298712903614)
(10, 0.167805983992305)
(11, 0.169121939493836)
(12, 0.166194620388966)
(13, 0.168251244207997)
(14, 0.16821098870929)
(15, 0.166778183814573)
(16, 0.167307098500703)
(17, 0.168424844336953)
(18, 0.167687162335992)
(19, 0.166749558387213)
(20, 0.166346549595281)
(21, 0.16743835099633)
(22, 0.167278276973729)
(23, 0.168081348491863)
(24, 0.169018673159691)
(25, 0.168021262002743)
(26, 0.167229642838772)
(27, 0.16693529028497)
(28, 0.166366613514394)
(29, 0.167083876277347)
(30, 0.16703243947603)
(31, 0.167509644234891)
(32, 0.167592497342523)
(33, 0.16673524671673)
(34, 0.167469610986336)
(35, 0.167778215920586)
(36, 0.167709637046308)
(37, 0.168686886004766)
(38, 0.16789535043204)
(39, 0.167535317514744)
(40, 0.165923741599232)
};


==> graphs/GreedyNP.k5C1.tex <==
\addplot [const plot,color=darkgreen,mark=asterisk,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 0.655984817943146)
(2, 0.514943469665143)
(3, 0.488050877295933)
(4, 0.483152484294689)
(5, 0.478675984240647)
(6, 0.478491886504277)
(7, 0.477680233723828)
(8, 0.476476354711527)
(9, 0.476718070496681)
(10, 0.476844634505642)
(11, 0.477734559338758)
(12, 0.474690422398261)
(13, 0.476160517040458)
(14, 0.475617515638963)
(15, 0.4768332177556)
(16, 0.47695849240052)
(17, 0.476679678005119)
(18, 0.47672631345663)
(19, 0.47669771731282)
(20, 0.476533289485913)
(21, 0.47629737129948)
(22, 0.476797803816155)
(23, 0.477941649568556)
(24, 0.476047155041143)
(25, 0.475947068537808)
(26, 0.47655473659377)
(27, 0.476740611528535)
(28, 0.477376875728308)
(29, 0.477505558375453)
(30, 0.47589702528614)
(31, 0.475403741805418)
(32, 0.477048020074493)
(33, 0.476540438521865)
(34, 0.476776356708298)
(35, 0.47526791012232)
(36, 0.47712665946997)
(37, 0.476518991414008)
(38, 0.476790654780203)
(39, 0.477720029454028)
(40, 0.476247328047813)
};


==> graphs/LPQ.k10C1.tex <==
\addplot [const plot,color=lightblue,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.841073164677409)
(3, 0.835629692700673)
(4, 0.850572529955755)
(5, 0.865712048749658)
(6, 0.878157545652113)
(7, 0.88975431014234)
(8, 0.898900459159241)
(9, 0.905854304138468)
(10, 0.912009534802969)
(11, 0.916907514450867)
(12, 0.921545997072402)
(13, 0.926034003903318)
(14, 0.928184052994051)
(15, 0.931309814224057)
(16, 0.933440918729241)
(17, 0.936903633787752)
(18, 0.937964422427381)
(19, 0.939972791668621)
(20, 0.942158840362152)
(21, 0.943584932213726)
(22, 0.945724069991087)
(23, 0.946671670497725)
(24, 0.948022704883426)
(25, 0.948773279542149)
(26, 0.950152460477553)
(27, 0.950706009288361)
(28, 0.952291598254914)
(29, 0.95316414129568)
(30, 0.953586339541211)
(31, 0.954271238917296)
(32, 0.955631655486232)
(33, 0.956082000281466)
(34, 0.955913120983253)
(35, 0.957010836421635)
(36, 0.957442416850401)
(37, 0.958314959891167)
(38, 0.958333724257635)
(39, 0.959271942581039)
(40, 0.959234413848102)
};


==> graphs/LPQ.k3C1.tex <==
\addplot [const plot,color=lightblue,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.888370377905498)
(3, 0.888396233319509)
(4, 0.902691811150927)
(5, 0.916764882742032)
(6, 0.9283045390105)
(7, 0.93689311643157)
(8, 0.944435771498565)
(9, 0.949949264789764)
(10, 0.95504734228744)
(11, 0.958259783613723)
(12, 0.962282502972009)
(13, 0.964816215761855)
(14, 0.967061733732003)
(15, 0.969847616989085)
(16, 0.971558773731042)
(17, 0.973023764064508)
(18, 0.974620843690335)
(19, 0.976019789377619)
(20, 0.976854353542995)
(21, 0.978379384463898)
(22, 0.979394070391585)
(23, 0.980288675144398)
(24, 0.981111231192286)
(25, 0.981513503128115)
(26, 0.982354071352234)
(27, 0.983308716692484)
(28, 0.983807053568212)
(29, 0.984029203741729)
(30, 0.984347418855146)
(31, 0.985230015490472)
(32, 0.9856322874263)
(33, 0.986064579655847)
(34, 0.986394802886751)
(35, 0.986887135703736)
(36, 0.987409488814439)
(37, 0.98775172016283)
(38, 0.987889813513935)
(39, 0.98812397180494)
(40, 0.988202024568608)
};


==> graphs/LPQ.k40C1.tex <==
\addplot [const plot,color=lightblue,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.801394137573182)
(3, 0.777996916125793)
(4, 0.787234786256073)
(5, 0.800678776125089)
(6, 0.812427760622423)
(7, 0.821282236683538)
(8, 0.828710470654996)
(9, 0.834688020895984)
(10, 0.842121534815018)
(11, 0.846313656811236)
(12, 0.849271332200422)
(13, 0.853578170585207)
(14, 0.856206458697965)
(15, 0.861598641206444)
(16, 0.865131917521529)
(17, 0.869174428377845)
(18, 0.868124517622845)
(19, 0.86983141539042)
(20, 0.871518726848676)
(21, 0.872929313715403)
(22, 0.874854242403457)
(23, 0.87627964401461)
(24, 0.879027418165606)
(25, 0.878737997256516)
(26, 0.882255105365134)
(27, 0.88284009464696)
(28, 0.884316650378067)
(29, 0.884558672244702)
(30, 0.885347369864893)
(31, 0.8858294042006)
(32, 0.8860542468196)
(33, 0.887151527620615)
(34, 0.890119498688429)
(35, 0.888696487047165)
(36, 0.890016630377012)
(37, 0.89070241911979)
(38, 0.890189960224935)
(39, 0.890618570840763)
(40, 0.892195857907009)
};


==> graphs/LPQ.k5C1.tex <==
\addplot [const plot,color=lightblue,mark=star,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 0.866412331644631)
(3, 0.867532715216243)
(4, 0.883379479357185)
(5, 0.898685761941736)
(6, 0.910289045525925)
(7, 0.919736201414946)
(8, 0.927522128326404)
(9, 0.934195468070497)
(10, 0.939730259300047)
(11, 0.944364998784481)
(12, 0.948551491406183)
(13, 0.951348723484876)
(14, 0.95445218945487)
(15, 0.957140916662496)
(16, 0.959250203748981)
(17, 0.961823875091151)
(18, 0.963075229305328)
(19, 0.965219940091079)
(20, 0.966835622216344)
(21, 0.967979467968744)
(22, 0.969666640453535)
(23, 0.97039584212069)
(24, 0.971811351239285)
(25, 0.972790769164778)
(26, 0.973612908299316)
(27, 0.974685263692191)
(28, 0.975843407516496)
(29, 0.975864854624354)
(30, 0.977130233987947)
(31, 0.977787945295577)
(32, 0.978216887452727)
(33, 0.979003281407502)
(34, 0.979803973434182)
(35, 0.979846867649897)
(36, 0.980819136539438)
(37, 0.98099786243825)
(38, 0.981491145918973)
(39, 0.981991578435648)
(40, 0.982313285053511)
};


==> graphs/OPTSort.k10C1.tex <==
\addplot [const plot,color=red,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
(31, 1)
(32, 1)
(33, 1)
(34, 1)
(35, 1)
(36, 1)
(37, 1)
(38, 1)
(39, 1)
(40, 1)
};


==> graphs/OPTSort.k3C1.tex <==
\addplot [const plot,color=red,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
(31, 1)
(32, 1)
(33, 1)
(34, 1)
(35, 1)
(36, 1)
(37, 1)
(38, 1)
(39, 1)
(40, 1)
};


==> graphs/OPTSort.k40C1.tex <==
\addplot [const plot,color=red,mark=x,mark size=2pt,mark repeat=2,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
(31, 1)
(32, 1)
(33, 1)
(34, 1)
(35, 1)
(36, 1)
(37, 1)
(38, 1)
(39, 1)
(40, 1)
};


==> graphs/OPTSort.k5C1.tex <==
\addplot [const plot,color=red,mark=x,mark size=2pt,mark repeat=4,smooth,line width=1pt] coordinates {
(1, 1)
(2, 1)
(3, 1)
(4, 1)
(5, 1)
(6, 1)
(7, 1)
(8, 1)
(9, 1)
(10, 1)
(11, 1)
(12, 1)
(13, 1)
(14, 1)
(15, 1)
(16, 1)
(17, 1)
(18, 1)
(19, 1)
(20, 1)
(21, 1)
(22, 1)
(23, 1)
(24, 1)
(25, 1)
(26, 1)
(27, 1)
(28, 1)
(29, 1)
(30, 1)
(31, 1)
(32, 1)
(33, 1)
(34, 1)
(35, 1)
(36, 1)
(37, 1)
(38, 1)
(39, 1)
(40, 1)
};

